Black holes in the limiting curvature theory of gravity

We discuss a recently proposed limiting curvature theory of gravity and its application to the problem of singularities inside black holes. In this theory the growth of the curvature is suppressed by specially chosen inequality constraints included in the gravity action. We consider a case of a spherically symmetric four dimensional black hole and demonstrated that imposed curvature constraints modify a solution in the black hole interior. Instead of forming the curvature singularity the modified metric describes a space which is exponentially expanding in one direction and oscillating the other two directions. The spacetime is complete and its polynomial curvature invariants are uniformly bounded.

==> REF.tex <==
@article{Volovich:1976aw,
    author = "Volovich, I. V. and Zagrebnov, V. A. and Frolov, Valeri P.",
    title = "{Quantum Production of Particles (The Hawking Effect) in Nonstationary Black Holes}",
    journal = "Teor. Mat. Fiz.",
    volume = "29",
    pages = "191--204",
    year = "1976"
}


@article{Markov1,
      author         = "Markov, M.A.",
      title          = "{Limiting density of matter as a universal law
of nature}",
      journal        = "JETP Letters",
      volume         = "36",
      pages          = "266",
      year           = "1982",
}

@article{Markov2,
      author         = "Markov, M.A.",
      title          = "{Problems of a Perpetually Oscillating Universe}",
      journal        = "Annals Phys.",
      volume         = "155",
      pages          = "333-357",
      doi            = "10.1016/0003-4916(84)90004-6",
      year           = "1984",
      SLACcitation   = "%%CITATION = APNYA,155,333;%%",
}

@article{FZ1,
    author = "Frolov, Valeri P. and Zelnikov, Andrei",
    title = "{Two-dimensional black holes in the limiting curvature theory of gravity}",
    eprint = "2105.12808",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "Alberta-Thy-17-21",
    doi = "10.1007/JHEP08(2021)154",
    journal = "JHEP",
    volume = "08",
    pages = "154",
    year = "2021"
}

@article{FZ2,
    author = "Frolov, Valeri P. and Zelnikov, Andrei",
    title = "{Bouncing cosmology in the limiting curvature theory of gravity}",
    eprint = "2108.09927",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "Alberta Thy 27-21",
    doi = "10.1103/PhysRevD.104.104060",
    journal = "Phys. Rev. D",
    volume = "104",
    number = "10",
    pages = "104060",
    year = "2021"
}

@article{FZ3,
    author = "Frolov, Valeri P. and Zelnikov, Andrei",
    title = "{Spherically symmetric black holes in the limiting curvature theory of gravity}",
    eprint = "2111.12846",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    reportNumber = "Alberta Thy 36-21",
    doi = "10.1103/PhysRevD.105.024041",
    journal = "Phys. Rev. D",
    volume = "105",
    number = "2",
    pages = "024041",
    year = "2022"
}

@inproceedings{FR,
    author = "Frolov, Valeri P.",
    title = "{Limiting curvature models of gravity}",
    booktitle = "{Quantum Gravity, Higher Derivatives \& Nonlocality}",
    eprint = "2111.14318",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    month = "11",
    year = "2021"
}

@article{Carballo-Rubio:2021wjq,
    author = "Carballo-Rubio, Ra\'ul and Di Filippo, Francesco and Liberati, Stefano and Visser, Matt",
    title = "{Geodesically complete black holes in Lorentz-violating gravity}",
    eprint = "2111.03113",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    month = "11",
    year = "2021"
}


